Light composite scalar in twelve-flavor QCD on the lattice

Based on lattice simulations using highly improved staggered quarks for twelve-flavor QCD with several bare fermion masses, we observe a flavor-singlet scalar state lighter than the pion in the correlators of fermionic interpolating operators. The same state is also investigated using correlators of gluonic interpolating operators. Combined with our previous study, that showed twelve-flavor QCD to be consistent with being in the conformal window, we infer that the lightness of the scalar state is due to infrared conformality. This result shed some light on the possibility of a light composite Higgs boson ("technidilaton") in walking technicolor theories.

==> table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{table}
  \begin{tabular}{c|c|r|l|l|l}
     $L^3 \times T$ & $m_f$ & \multicolumn{1}{|c}{$N_{\rm cfgs}$} & \multicolumn{1}{|c|}{$m_\sigma$} & \multicolumn{1}{c}{$m_\pi$} & \multicolumn{1}{|c}{$m_\sigma/m_\pi$}\\
     \hline
     $24^3 \times 32$ & 0.05 &11000 & 0.237(13)($^{02}_{01}$) & 0.3273(19)$^*$ & 0.73(4)($^{1}_{0}$) \\
     $24^3 \times 32$ & 0.06 & 14000 & 0.279(17)($^{07}_{01}$) & 0.3646(16)$^*$ & 0.77(5)($^{2}_{0}$) \\
     $24^3 \times 32$ & 0.08 & 15000 & 0.359(21)($^{01}_{18}$) & 0.4459(11)& 0.81(5)($^{0}_{4}$) \\
     $24^3 \times 32$ & 0.10 &  9000 & 0.453(42)($^{37}_{08}$) & 0.5210(7) & 0.87(8)($^{7}_{2}$) \\
     $30^3 \times 40$ & 0.05 & 10000 & 0.275(13)($^{21}_{08}$) &  0.3192(14)$^*$ & 0.86(4)($^{7}_{3}$)\\
     $30^3 \times 40$ & 0.06 & 15000 & 0.329(15)($^{47}_{12}$) & 0.3648(9)$^*$ & 0.90(4)($^{13}_{3}$)\\
     $30^3 \times 40$ & 0.08 & 15000 & 0.382(21)($^{03}_{16}$) & 0.4499(8) & 0.85(5)($^{1}_{4}$)\\
     $30^3 \times 40$ & 0.10 &  4000 & 0.431(51)($^{06}_{04}$) & 0.5243(7) & 0.82(10)($^{1}_{1}$)\\
     $36^3 \times 48$ & 0.05 &  5000 & 0.283(23)($^{01}_{02}$) & 0.3204(7)$^*$ & 0.88(7)($^{0}_{1}$)\\
     $36^3 \times 48$ & 0.06 &  6000 & 0.305(22)($^{25}_{06}$) & 0.3636(9)$^*$ & 0.84(6)($^{7}_{2}$)\\
   \end{tabular}
   \caption{\label{tab:simulations} Parameters of lattice simulations for $N_f=12$ QCD at fixed $\beta=4.0$. $N_{\rm cfgs}$ is the number of saved gauge configurations. The second error of $m_\sigma$ is a systematic error coming from the fit range. The values of $m_\pi$ are from Ref.~\cite{Aoki:2012eq}, but the ones with ($^*$) have been updated. The error on $m_\sigma/m_\pi$ comes only from $m_\sigma$.}
 \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

